Measurement of inclusive jet charged-particle fragmentation functions in Pb+Pb collisions at $\sqrt{s_{NN}} = 2.76$ TeV with the ATLAS detector

Measurements of charged-particle fragmentation functions of jets produced in ultra-relativistic nuclear collisions can provide insight into the modification of parton showers in the hot, dense medium created in the collisions. ATLAS has measured jets in $\sqrt{s_{NN}} = 2.76$ TeV Pb+Pb collisions at the LHC using a data set recorded in 2011 with an integrated luminosity of 0.14 nb$^{-1}$. Jets were reconstructed using the anti-$k_{t}$ algorithm with distance parameter values $R$ = 0.2, 0.3, and 0.4. Distributions of charged-particle transverse momentum and longitudinal momentum fraction are reported for seven bins in collision centrality for $R=0.4$ jets with $p_{{T}}^{\mathrm{jet}}> 100$ GeV. Commensurate minimum $p_{\mathrm{T}}$ values are used for the other radii. Ratios of fragment distributions in each centrality bin to those measured in the most peripheral bin are presented. These ratios show a reduction of fragment yield in central collisions relative to peripheral collisions at intermediate $z$ values, $0.04 \lesssim z \lesssim 0.2$ and an enhancement in fragment yield for $z \lesssim 0.04$. A smaller, less significant enhancement is observed at large $z$ and large $p_{\mathrm{T}}$ in central collisions.

==> auxiliaryPlots.tex <==
\onecolumn
\clearpage
\section{\Large Auxiliary plots}

\begin{figure*}[h]
\centerline{
\includegraphics[width=0.8\textwidth]{p113_Unfolding_v1_diff1c.pdf}
}
\caption{
  Left: The difference in unfolded distributions between \mbox{0--10\%} central and 
\mbox{60--80\%} peripheral collisions, $\Delta\Dz$ (top), $\Delta\Dpt$ (bottom) 
respectively. Right: The unfolded fragmentation functions evaluated in the 
extended $z$-range of $z$=0.01--1 for \mbox{0--10\%} central and \mbox{60--80\%} peripheral 
collisions, $D_{ext}(z)$ (top), and the corresponding central-to-peripheral 
ratio, $R_{D_{ext}(z)}$ (bottom). All distributions are evaluated for 
\RThree\ jets.
}
\label{fig:diff}
\end{figure*}



\begin{figure*}
\centerline{
\includegraphics[width=0.45\textwidth]{DzAll_R2_un10r9.pdf}
\includegraphics[width=0.45\textwidth]{DPtAll_R2_un10r9.pdf}
}
\vspace{-0.15in}
\caption{
Unfolded \RTwo\ longitudinal charged particle fragmentation functions,
\Dz\ and \Dpt, for the seven centrality bins included in this analysis. The
statistical uncertainties are everywhere smaller than the points. The shaded
error bars indicate systematic uncertainties.
Grey lines connecting the central values of distributions are to guide the eye.
}
\label{fig:dpttwo}
\end{figure*}



\begin{figure*}
\centerline{
\includegraphics[height=3.5in]{p113_Unfolding_v1_z3nr_ca{ehv+eiv}_un9r9_sr.pdf}
}
\vspace{-0.15in}
\caption{
Ratios of \Dz\ for six bins in collision
centrality to those in peripheral (\mbox{60--80\%}) collisions, \Dzratio, for
\RThree\ jets. The error bars on the data points indicate statistical
uncertainties while the shaded bands indicate systematic uncertainties that
are uncorrelated or partially correlated between points. 
}
\label{fig:dzratiorthree}
\end{figure*}


\begin{figure*}
\centerline{
\includegraphics[height=3.5in]{p113_UnfoldingPt_v1_z3nr_ca{ehv+eiv}_un9r9_sr.pdf}
}
\vspace{-0.15in}
\caption{
Ratios of \Dpt\ for six bins in collision
centrality to those in peripheral (\mbox{60--80\%}) collisions, \Dptratio, for
\RThree\ jets. The error bars on the data points indicate statistical
uncertainties while the shaded bands indicate systematic uncertainties that
are uncorrelated or partially correlated between points.
}
\label{fig:dptratiorthree}
\end{figure*}



\begin{figure*}
\centerline{
\includegraphics[height=3.5in]{p113_Unfolding_v1_z3nr_ca{fhv+fiv}_un9r9_sr.pdf}
}
\vspace{-0.15in}
\caption{
Ratios of \Dz\ for six bins in collision
centrality to those in peripheral (\mbox{60--80\%}) collisions, \Dzratio, for
\RTwo\ jets. The error bars on the data points indicate statistical
uncertainties while the shaded bands indicate systematic uncertainties that
are uncorrelated or partially correlated between points. 
}
\label{fig:dzratiortwo}
\end{figure*}


\begin{figure*}
\centerline{
\includegraphics[height=3.5in]{p113_UnfoldingPt_v1_z3nr_ca{fhv+fiv}_un9r9_sr.pdf}
}
\vspace{-0.15in}
\caption{
Ratios of \Dpt\ for six bins in collision
centrality to those in peripheral (\mbox{60--80\%}) collisions, \Dptratio, for
\RTwo\ jets. The error bars on the data points indicate statistical
uncertainties while the shaded bands indicate systematic uncertainties that
are uncorrelated or partially correlated between points. 
}
\label{fig:dptratiortwo}
\end{figure*}



\begin{figure*}
\centerline{
\includegraphics[height=3.5in]{p113_UnfoldingKsi_v1_z3nr_ca{dhv+div}_un9r9_sr.pdf}
}
\vspace{-0.15in}
\caption {
  Ratios of $D(\xi)$ distributions for six bins in collision centrality to those 
in peripheral (\mbox{60--80\%}) collisions, $R_{D(\xi)}$, for \RFour\ jets. $D(\xi)$ 
distributions were recalculated from original $D(z)$ distributions based on the 
relation $\xi = \ln(1/z)$. The error bars on the data points indicate statistical 
uncertainties while the shaded bands indicate systematic uncertainties that are 
uncorrelated or partially correlated between points.
  }
\label{fig:dxiratiortwo}
\end{figure*}

